Efficient-Empathy: Towards Efficient and Effective Selection of Empathy Data

In recent years, with the rapid advancements in large language models (LLMs), achieving excellent empathetic response capability has become a crucial prerequisite. Consequently, managing and understanding large-scale video datasets has gained increasing importance. However, empathetic data are typically trained without any quality selection, leading to inefficient data usage and wasted computational resources. Additionally, using raw data can result in low performance in empathetic dialogues. In this work, we present Efficient-Empathy, a sensibility and rationality score-based data selection algorithm that automatically selects sensibility and rationality data while discarding low-quality data. With only the sensibility data (59% of the full dataset), our trained sensibility model efficiently achieves state-of-the-art (SoTA) performance. Furthermore, with multiple data selection hyperparameters, the sensibility model demonstrates SoTA performance, showcasing the robustness of our method. By integrating sensibility and rationality data with a MoE structure, we achieve even higher performance, demonstrating the effectiveness of our Efficient-Empathy algorithm.

==> table/human_eval.tex <==
\begin{table}[htbp]
  \centering
  \caption{Results of human evaluation.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cccc}
    \toprule
    \textbf{Models} & \textbf{Coh.} & \textbf{Emp.} & \textbf{Inf.} & \textbf{Cont.} \\
    \midrule
    SEEK  &	-  &	-  &	-  &	- \\
    KEMP  &	-  &	-  &	-  &	- \\
    DCKS  &	-  &	-  &	-  &	- \\
    Qwen1.5-1.8B-Chat &	-  &	-  &	-  &	-\\
    LLaMA3-8B-Chat	&	-  &	-  &	-  &	- \\
    Qwen1.5-72B-Chat	&	-  &	-  &	-  &	- \\
    \textbf{Ours} &	-  &	-  &	-  &	- \\
    \bottomrule
    \end{tabular}%
 }
  \label{tab:huamn_exp}%
\end{table}%

==> table/moe-structure.tex <==
% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table*}[htbp]
%   \centering
%   \caption{Moe structere parameters}
%   \resizebox{\linewidth}{!}{
%     \begin{tabular}{lllll}
%     \toprule
%     \textbf{MoE-Architecture} & \textbf{Shared Expert} & \textbf{Activated Experts} & \textbf{Routing Method} & \textbf{FT Method} \\
%     \midrule
%     a     & Qwen1.5-1.8B-Chat & Sensibliety-2, Rationality-2 & Soft routing & Full-parameter \\
%     b     & Rationality-2 & Sensibility-2, Discard-2 & Soft routing & Full-parameter \\
%     c     & None  & Sensibliety-2, Rationality-2 & None  & Full-parameter \\
%     d     & None  & LLaMA3-8B-Instruct, Sensibility, Rationality & Soft routing & Router parameters only \\
%     e     & None  & Sensibliety-2, Rationality-2 & Top-1 routing & Router parameters only \\
%     f     & None  & Sensibliety-2, Rationality-2 & Top-1 routing & Router parameters only \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:moe-structure}%
% \end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Moe structere parameters}
    \begin{tabular}{lllll}
    \toprule
    \textbf{MoE-Architecture} & \textbf{Seed Model} & \textbf{Expert-1} & \textbf{Expert-2} & \textbf{Routing Method} \\
    \midrule
    a     & LLaMA3-8B-Instruct & Sensibilit Expert  w/ $D_s$ & LLaMA3-8B-Instruct & Soft routing \\
    b     & LLaMA3-8B-Instruct & Sensibilit Expert  w/ $D_s$ & Discard w/ $D_n$ & Soft routing \\
    c     & Qwen1.5-1.8B-Chat & Sensibilit Expert  w/ $D_s$ & Rationality Expert w/ $D_r$ & Soft routing \\
    d     & Qwen1.5-1.8B-Chat & Sensibilit Expert  w/ $D_s$ & Qwen1.5-1.8B-Chat & Soft routing \\
    e     & Qwen1.5-1.8B-Chat & Sensibilit Expert  w/ $D_s$ & Discard w/ $D_n$ & Soft routing \\
    f     & LLaMA3-8B-Instruct & Sensibilit Expert  w/ $D_s$ & Rationality Expert w/ $D_r$ & Top-1 routing \\
    \bottomrule
    \end{tabular}%
  \label{tab:moe-structure}%
\end{table*}%

